CHAD for Expressive Total Languages

We show how to apply forward and reverse mode Combinatory Homomorphic Automatic Differentiation (CHAD) to total functional programming languages with expressive type systems featuring the combination of - tuple types; - sum types; - inductive types; - coinductive types; - function types. We achieve this by analysing the categorical semantics of such types in $\Sigma$-types (Grothendieck constructions) of suitable categories. Using a novel categorical logical relations technique for such expressive type systems, we give a correctness proof of CHAD in this setting by showing that it computes the usual mathematical derivative of the function that the original program implements. The result is a principled, purely functional and provably correct method for performing forward and reverse mode automatic differentiation (AD) on total functional programming languages with expressive type systems.

==> App-Concrete-Model.tex <==
\section{A Concrete Model: Sets and Families of Commutative Monoids}\label{sec:concrete-model}
\mv{Describe the concrete semantics we have in mind here --
$\catC=\Set$, $\catC'=\Fam{\Set}$, $\catL=\Fam{\CMon}$.
I don't think anything will be surprising, except the 
calculation of inductive and coinductive types in $\catL$.
The real question is what those look like.
Presumably they exist because $\CMon$ is locally presentable.
I think it'd be good to start with an example -- the induced 
tangent and cotangent spaces to lists of real numbers.
Then, if you understand that, proceed to binary trees.
Then, perhaps see if you can do streams of real numbers (for a coinductive type).
Then, perhaps see if there  is a general formula.
(I would hope that CHAD ends up computing the (co)tangent spaces that you would 
expect -- the (co)tangent space to the type of lists of reals, at a list of length n, is an
n-dimensional vector.
Does that suggest that the canonical morphism
between the inductive and coinductive types in the fibres is an iso
for the functors we consider?
So we have some notion of algebraic compactness in the fibres (for our class of functors)?)
}
\begin{equation*}
	\begin{tikzpicture}[x=3cm, y=2cm]
		\node (a) at (0,0) {$A $};
		\node (b) at (1, 0) { $B$ };
		\node (c) at (1,-1) {$\mathsf{2}\otimes B $};
		\node (d) at (0,-1) {$ B $};
		\draw[->] (a)--(b) node[midway,above] {$ p  $};
		\draw[->] (b)--(c) node[midway,right] {$ \nu _1  $};
		\draw[->] (a)--(d) node[midway,left] {$ p  $};
		\draw[->] (d)--(c) node[midway,below] {$ \nu _0  $};
		\draw[double,->] (0.3,-0.6)--(0.7,-0.6) node[midway,above] {$\alpha\ast \id _ p $};
	\end{tikzpicture} 
\end{equation*}   

\begin{equation*}
	\begin{tikzpicture}[x=3cm, y=2cm]
		\node (a) at (0,0) {$A $};
		\node (b) at (1, 0) { $B$ };
		\node (c) at (1,-1) {$\mathsf{2}\otimes B $};
		\node (d) at (0,-1) {$ B $};
		\draw[->] (a)--(b) node[midway,above] {$ p  $};
		\draw[->] (b)--(c) node[midway,right] {$ \nu _1  $};
		\draw[->] (a)--(d) node[midway,left] {$ p  $};
		\draw[->] (d)--(c) node[midway,below] {$ \nu _0  $};
		\draw[double,->] (0.3,-0.6)--(0.7,-0.6) node[midway,above] {$\alpha\ast \id _ p $};
	\end{tikzpicture} 
\end{equation*}   

==> App-Coproducts_total_category.tex <==
\section{Coproducts in the total category}


==> App-Fibrations_and_indexed_categories.tex <==
\section{Fibrations and indexed categories}
 




==> App-Indexedcategories_respecting.tex <==
\section{Preservation, reflection and creation of initial algebras}\label{sect:appendix-has-inductive-types}





==> App-Initial_algebras_split_fibrations.tex <==
\section{Parameterized initial algebras for split fibrations}

==> App-MuPolynomials.tex <==
\section{$\mu$-Polynomials}\label{sec:appendix-MuPolynomials}
The positive types of our source language $\Syn $ consist of the initial algebras (inductive types)
of the so called $\mu$-polynomials. For this reason, we recall below the definition and 

==> App-Terminal_Coalgebras_split_fibrations.tex <==
\section{Parameterized terminal coalgebras for split fibrations}\label{sect:appendix-coinductivetypes-grothendieckconstruction}


==> changes <==
Summary of changes we made:
- added table of contents
- added extra citations throughout to relate more to revevant work
- explained connections to differential geometry of manifolds more in key ideas section
- added section 2.6 summarising a strengthened version of the correctness theorem, relating to derivatives of functions between manifolds
- fixed typos and made minor rewrites throughout
- incorporated most appendices into the main text; the remaining ones are truly optional and should not be in the main text;
- improved formatting in section 8, to made AD code transformations easier to read
- simplified the AD correctness proofs (section 12) to no longer depend on Boman's theorem; as a consequence they now apply more generally to plain differentiable functions rather than merely smooth (C^\infty) functions 
- added section 13 detailing our strengthened correctness theorem that shows that the AD transformations even calculate correct derivatives in the differential geometry sense for functions whose global inputs and outputs are are types constructed from real numbers, tuples, variant types, type variables and inductive type formers;
- added an interesting example of a program with inductive types and variant types that we differentiate: an evaluator for polynomial expressions
- added some more context in main text of paper to make it easier to read independently of section 2


Major criticisms by reviewers and the way we addressed them:
- Reviewer 1: paper is very long; appendices -> main text; split up paper?
    We have decided not to split up the paper as it might be hard to keep the story coherent that way. We have moved the appendices into the main text where appropriate.
- Reviewer 1: : 1. What about the ring structure of R? Why are we only interested in the commutative monoid structure? In
classical calculus, the derivative is not only a monoid morphism but an R-linear morphism. This should be
addressed. Possibly in the introduction (say page 4), or later on.
    Thank you for the suggestion! We have added a footnote (footnote a) to discuss this phenomenon.
- Reviewer 1: Regarding the paragraph after Theorem 9, the one discussing the major difference between exponentials and
the other types. Would it be interesting to know when this is the case? What goes wrong? What conditions do
we need to make it work?
    Agreed. This is an interesting question. We address it in our forthcoming work about symmetric monoidal closure of total categories of Grothendieck constructions, where 
    we generalize the construction of exponentials in this paper to encompass more general Dialectica/Diller-Nahm like constructions. We show that the exponentials we get in \Sigma_\catC \catL are fibred precisely if \catL has an indexed symmetric monoidal closed structure.
    This is beyond the scope of the current paper.
- Reviewer 2: examples 
    We have added a compelling example program that uses inductive types and variant types to represent polynomials. We write an evaluator for such polynomials and calculate its derivative.
- Reviewer 2: cut and paste major explanations from key ideas section into main text
    We have decided against this and have instead polished the key ideas section further and ensured to make the main text easier to read and less technical. Our decision was motivated by our view that a 100 page paper needs a key ideas section that can be read independently to help the reader understand the points of the paper without having to read the full thing.
- Reviewer 2: give full definitions of denotational semantics for source and target languages in appendix
    We have added section 10.3 that describes these semantics.

==> response <==
Dear Reviewers,

We are writing to express our gratitude for the detailed and insightful feedback provided on our paper and to explain how we have revised it based on your suggestions. We appreciate the time and effort you have invested in providing thoughtful suggestions for improvement. We are pleased to inform you that we have revised the manuscript in light of your feedback, and we believe that the paper has been improved a lot as a result.

We have made the following changes to the manuscript:
- Added a table of contents to provide a clearer overview of the paper's structure.
- Incorporated additional citations throughout the text to better situate our work in relation to relevant prior work.
- Provided more detailed explanations of the connections between our work and the differential geometry of manifolds in the key ideas section.
- Added a new section (2.6) that summarizes a strengthened version of the correctness theorem, focusing on the derivatives of functions between manifolds.
- Corrected typos and made minor rewrites throughout the manuscript.
- Incorporated most appendices into the main text where appropriate.
- Improved formatting in section 8 to make the automatic differentiation (AD) code transformations easier to read.
- Simplified the AD correctness proofs in section 12 to remove reliance on Boman's theorem, thus allowing the results to apply more generally to plain differentiable functions rather than just smooth (C^\infty) functions.
- Added a new section (13) detailing a strengthened correctness theorem that demonstrates that the AD transformations even calculate correct derivatives in the differential geometry sense for functions whose global inputs and outputs are types constructed from real numbers, tuples, variant types, type variables, and inductive type formers.
- Added a examples of programs with inductive types and variant types that we differentiate: an evaluator for polynomial expressions; sum of elements of a list; multiplication of elements of a list.
- Provided additional context in the main text to make it easier to read independently of section 2.


We have also addressed the following specific criticisms from the reviewers:

Reviewer 1:
Criticism: The paper is very long; appendices should probably be moved into the main text and you could consider splitting the paper up.
Response: We have moved most of the appendices into the main text where appropriate and kept the paper as a single coherent piece to maintain the overall structure of the argument.
Criticism: The paper does not address the ring structure of R and its implications for the differentiation process.
Response: We have added a footnote discussing this phenomenon (footnote a on page 7).
Criticism: The paragraph after Theorem 9 discussing the differences between exponentials and other types (exponentials not being fibred) should be expanded upon.
Response: We acknowledge this is an interesting question. We address it in our forthcoming work about symmetric monoidal closure of total categories of Grothendieck constructions, where we generalize the construction of exponentials in this paper to encompass more general Dialectica/Diller-Nahm like constructions. We show that the exponentials we get in $\Sigma_C L$ are fibred precisely if $L$ has an indexed symmetric monoidal closed structure. This is beyond the scope of the current paper.

Reviewer 2:
Criticism: The paper lacks examples.
Response: We have added an example program that uses inductive types and variant types to represent polynomials. We write an evaluator for such polynomials and calculate its derivative.
Criticism: The major explanations from the key ideas section should perhaps be cut and pasted into the main text to make the main text easier to read.
Response: We have decided to keep the key ideas section separate and instead made the main text more accessible to readers. The key ideas section provides a helpful overview of the paper's core concepts and can be read independently of the main text, which we believe is important for a 100+ page paper.
Criticism: The paper lacks full definitions of denotational semantics for source and target languages.
Response: We have added a new section (10.3) that describes these semantics in detail.

Once again, we would like to express our gratitude for the valuable feedback provided by the reviewers. We believe that their input has significantly improved the quality and clarity of the paper, and we hope that they are happy with our revisions.

Kind regards,
Fernando and Matthijs

==> reviews <==
Reviewer(s)' Comments to Author:
Referee: 1

Comments to the Author
I recommend this paper be accepted, pending the minor corrections made in my full attached review. This paper is well written and is already very polished. The proofs are well done, easily to follow, and I found no mathematical errors. The only potential point of concern is the length of the paper, which is almost 100 pages, including almost 20 pages of appendix. Such a long paper could be intimidating for any new reader. On the other hand, this paper provides a complete story. Due to the length of the paper, an argument could be made to not have an appendix, and move the appendix sections into the main part (at the appropriate locations). Another argument could be made to split the paper into two parts: one part on the more theoretical category theory story, and another part on the rest. But again, I understand the authors' idea of having one complete story in one paper. I leave this discussion to the authors and the editorial board. Nevertheless, overall this is a very good paper, on a very popular and current area of research, and will surely help push forward said area. In the attached review I have a list of minor comments such as typos and formatting suggestions to be fixed.

Referee: 2

Comments to the Author
\1. Summary:

The authors of CHAD for Expressive Total Languages use categorical semantics to determine the forward and reverse mode Automatic Differentiation (AD) transformations of a total functional programming language with expressive types including tuple, sum, inductive and coinductive types. They show that their forward and reverse mode transformations are correct in the sense that any term with real input and output types in the source language is transformed to its derivative and transposed derivative respectively. This theoretical work lays the groundwork for an implementation of forward and reverse mode AD on expressive programming languages.

The main contributions are as follows:
Develop an abstract categorical semantics for the source language, a total functional language with expressive types
Present the target language for the AD transformation
Define the forward and reverse mode AD transformation on the source language
Design a novel categorical logical relation to prove the correctness of the AD transformation.

\2. Evaluation:

Pros:
As far as I am aware, this is the first paper to define a reverse mode AD on an expressive functional language.
The AD transformation on sum, inductive and coinductive types are new and interesting.
The categorical arguments given are involved but well-presented. The enquiry is thorough.
The results of the paper demonstrate the expressiveness of the categorical semantics.

Cons:
Insights to the definitions of the source and target languages and the AD transformations are given in Section 2 but not when the definitions are stated in the later sections. It is troublesome to refer back to Section 2 for insights when the definitions are presented.
Not many examples are given in the paper to illustrate the workings of the transformation on the extended language. Since this is the first paper to consider reverse mode AD transformation on expressive types, I think examples are essential.
The denotational semantics for the source and target languages are not stated in full. For completeness, they should be included in the main paper or in the Appendix.


\3. Major comments:
As mentioned above, I think the paper is novel and thorough in its exploration of AD transformations on functional languages with expressive type systems. Section 2 was very helpful in giving insights to how the AD transformation is defined on sum, inductive and coinductive types, though I would prefer them to be located with the definitions in the later sections.

Suggestions:
Present the denotational semantics for the source and target languages
Give more examples to illustrate the AD transformations on the source language
Cut and paste the insights into the relevant sections instead of in Section 2

\4. Minor comments | typos

p4
reverse mode primal values D(\tau)_2 → D(\tau)_1
Use =^{def} for definition

p5
D(\bar{\Gamma})t → D_{\bar{\Gamma}}t
Reverse mode AD:
D(\Gamma)_1 \vdash D_{\bar{\Gamma}}t : D(\sigma)*(D(\Gamma)_2 \multimap D(\sigma))
→ D(\Gamma)_1 \vdash D_{\bar{\Gamma}}t : D(\sigma)*(D(\sigma) \multimap D(\Gamma)_2)
D_{\bar{\Gamma}}() =^{def} … in <, \lambda v.x’ \cdot (fst v)>+y’ \cdot (snd v)
→ D_{\bar{\Gamma}}() =^{def} … in <, \lambda v.x’ \cdot (fst v)+y’ \cdot (snd v)>

p15
Definition 3. Let D be a category *with* $\mu \nu$-polynomials. …

p18
(Fig 5) It is unclear \Rightarrow means imply

p19
objects are pairs (A_1, A_2) of an object … and an object A_2 of L(A_2)
→ objects are pairs (A_1, A_2) of an object … and an object A_2 of L(A_1)
Either use ; or \circ for composition of functions

p36
For all op \in Op^{m_1,\dots, m_r}_{n_1,\dots, n_k}
→ For all op \in Op^{m}_{n_1,\dots, n_k}

p38
(Fig 7: caption) kinding context \Gamma can be used as a linear type … → kinding context \Delta can be used as a linear type … (?)

p39 (Fig 8)
Typing rule for linear let: Shouldn’t the unique linear identifier v be in the typing context?
Typing rule for copower elimination: Why is a kinding judgment for the linear type \pho’ included? Is it not implicit that it is well-kinded?

p49
following corollary by Corollary the universal property …
→ following corollary by the universal property …

p52
FSet → FLi

p58
\underline{\hat{G}}_{\gamma}:E’-Alg \to E-Alg
→ \underline{\hat{G}}_{\gamma}:E-Alg \to E’-Alg

p64
(Lemma 63) The category D is not defined but it should be Set.
(Lemma 63) The codomain of forward and reverse pi should be Set x Fam(Vect) and Set x Fam(Vect^{op})
